Fairness and Bias in Truth Discovery Algorithms: An Experimental Analysis

Machine learning (ML) based approaches are increasingly being used in a number of applications with societal impact. Training ML models often require vast amounts of labeled data, and crowdsourcing is a dominant paradigm for obtaining labels from multiple workers. Crowd workers may sometimes provide unreliable labels, and to address this, truth discovery (TD) algorithms such as majority voting are applied to determine the consensus labels from conflicting worker responses. However, it is important to note that these consensus labels may still be biased based on sensitive attributes such as gender, race, or political affiliation. Even when sensitive attributes are not involved, the labels can be biased due to different perspectives of subjective aspects such as toxicity. In this paper, we conduct a systematic study of the bias and fairness of TD algorithms. Our findings using two existing crowd-labeled datasets, reveal that a non-trivial proportion of workers provide biased results, and using simple approaches for TD is sub-optimal. Our study also demonstrates that popular TD algorithms are not a panacea. Additionally, we quantify the impact of these unfair workers on downstream ML tasks and show that conventional methods for achieving fairness and correcting label biases are ineffective in this setting. We end the paper with a plea for the design of novel bias-aware truth discovery algorithms that can ameliorate these issues.

==> discussion.tex <==
\section{Discussion}
\label{sec:discussion}

\begin{itemize}
    \item CrowdWorkSheets: see paper
\end{itemize}

To the best of our knowledge, 
only one paper addressed fairness issues in a crowdsourcing setting proposing 
a new truth discovery algorithm that takes into account the sensitive features of the samples \cite{kdd2020}.
While the authors proposed three pre-, in-, and post-processing approaches 
to mitigate the bias of the true inference, they mainly focused on the statistical parity notion of fairness, 
which is very sensitive to the behavioral bias of the different groups represented in the data.
Furthermore, to address the challenges of collecting and 
aggregating trustworthy labels from multiple annotators, 
there is still much room for further research and improvement.
